Characterizing Direct Product Testing via Coboundary Expansion

A $d$-dimensional simplicial complex $X$ is said to support a direct product tester if any locally consistent function defined on its $k$-faces (where $k\ll d$) necessarily come from a function over its vertices. More precisely, a direct product tester has a distribution $\mu$ over pairs of $k$-faces $(A,A')$, and given query access to $F\colon X(k)\to\{0,1\}^k$ it samples $(A,A')\sim \mu$ and checks that $F[A]|_{A\cap A'} = F[A']|_{A\cap A'}$. The tester should have (1) the ``completeness property'', meaning that any assignment $F$ which is a direct product assignment passes the test with probability $1$, and (2) the ``soundness property'', meaning that if $F$ passes the test with probability $s$, then $F$ must be correlated with a direct product function. Dinur and Kaufman showed that a sufficiently good spectral expanding complex $X$ admits a direct product tester in the ``high soundness'' regime where $s$ is close to $1$. They asked whether there are high dimensional expanders that support direct product tests in the ``low soundness'', when $s$ is close to $0$. We give a characterization of high-dimensional expanders that support a direct product tester in the low soundness regime. We show that spectral expansion is insufficient, and the complex must additionally satisfy a variant of coboundary expansion, which we refer to as \emph{Unique-Games coboundary expanders}. Conversely, we show that this property is also sufficient to get direct product testers. This property can be seen as a high-dimensional generalization of the standard notion of coboundary expansion over non-Abelian groups for 2-dimensional complexes. It asserts that any locally consistent Unique-Games instance obtained using the low-level faces of the complex, must admit a good global solution.

==> old.tex <==
\subsubsection{Proof of Lemma~\ref{lem:core-jump} with $T$ dependent on $R$}
Fix $R, t, T$ as in Lemma~\ref{lem:core-jump}. Without loss of generality, we can assume that $f$ is the all $0$'s function and use $\cB$ to denote $\cB_R(0)$.

\begin{lemma}[Lemma~\ref{lem:core-jump} restated]
Let $R \in (0,1)$ with $R = \Theta(t/k)$, $T > 2(t + kR)$. Suppose for all functions $g \in \cB_R(0)$ it holds that $\agr_T(g, G) < \delta-\delta^{18}$ then,
\[\Pr_{s \sim \cC(d/2)}[\forall f \in \cB: \agr_t(f|_s, G|_s) < \delta - \frac{\delta^{18}}{2}] > 1 - o(1).\]
\end{lemma}


\begin{proof}
Let $\cR = \Agr_T(0)$. For all $g \in \cB$ write:
\[\Agr_{t}(g) = A_1(g) \sqcup A_2(g),\]
where $A_1(g) = \Agr_{t}(g) \cap \cR$ and $A_2(g) = \Agr_{T}(g) \setminus \cR$. Firstly by sampling we get that, $|\Agr_T(0)| = \agr_T(0) \approx \agr_T(0|_s, G|_s)$:
\[\Pr_{s \sim X(d/2)}[\agr_T(0|_s, G|_s) \leq \agr_T(0,G)+\delta^{100}] \geq 1-o(1).\]
This immediately bounds $|A_1(g)|_s|$ by $\delta - \delta^{18}+\delta^{100}$, since $A_1(g)|_s \subseteq \Agr_T(0)|_s$ and the latter is bounded by $\delta-\delta^{18}+\delta^{100}$.

We can now bound $|A_2(g)|_s|$ to complete the proof.
Every $A \in A_2(g)|_s$ satisfies $\Delta_A(g,0) > 4R$. Assume for the sake of contradiction that this is not the case. Then by the triangle inequality we get $\Delta(F[A],0) \leq \Delta_A(F[A],g[A]) + \Delta_A(g,0) \leq t + 4r < T$, by the assumption in the lemma. But since $A_2(g) \cap \Agr_T(0) = \phi$ by definition, this is a contradiction. We can now upper bound the fraction of $k$-sets in $A \subset s$ that have $\Delta_A(g,0) > 4R$. We know that $\Delta_s(g, 0) < 2R$ since $s \in X(d/2)$. By a Chernoff bound (similar to that in Claim~\ref{claim:dist-vs-agr}) we get that:
\[\Pr_{A \sim \cC_s(k)}[\Delta_A(g,0) > 4R] \leq \exp(-Rk) \leq \delta^{40}.\]
Hence this gives us that $|A_2(g)|_s| \leq \delta^{40}$ for all $s \in X(d/2)$ and $g \in \cB_R(0)$. Combining this with the bound for $|A_1(g)|_s|$ completes the proof.

%Since ${A_2(g) \subseteq \Agr_T(g) \setminus \Agr_T(g|_C)}$ we get that $A_2(g) \leq \delta^{40}$. Therefore after randomization $\Agr_T(g) \leq \delta^{40}$ for all $g$. Therefore the $\beta$-agreement test for $\beta = 1/t$ passes w.p. $\leq \delta^{20}$ globally. Therefore on most $s$, all functions satisfy $\agr_t(f) \leq \delta^{10}$. This implies that $A_2(g) \cap \Agr_t(g)$ jumps to at most $\delta^{10}$, and $A_1(g) \cap \Agr_t(g)$ jumps to at most $\delta-\delta^5+\delta^{100}$ therefore $\agr_t(g)$ on most $s$ is at most $\delta$.
\end{proof}







\begin{lemma}[Agreement sets do not jump]
W.p. at least $1- 1/k^{10}$ on $\cC(d(1-\beta))$, the size of every agreement set (corresponding to a global function on $[d]$) changes by an additive factor of at most $1/k^{10}$, when $d \ll k^{11}$ and $\beta \leq 1/k^2$. 
\end{lemma}

\begin{proof}
We will ``cover'' the agreement sets of the global functions, i.e. we will find sets $S_1, \ldots, S_{m} \subseteq \cC(k)$ with $m \leq k^{11}$, such that $|\Agr_\eta(f) \setminus \cup S_i| \leq 1/k^{11}$. 

\paragraph{Small cover:} 
We iteratively build a family of sets $\cS$ as required via the following algorithm:
\begin{enumerate}
\item Initialize $\cS = \phi$. 
\item While there exists $f$ on $[d]$ such that $|\Agr_\eta(f) \setminus \cup_{S \in \cS} S| > 1/k^{11}$:
\begin{enumerate}
    \item Choose an arbitrary such function $f$.
    \item $\cS \leftarrow \cS \cup (\Agr_\eta(f) \setminus \cS)$. 
\end{enumerate}
\item Output $\cS$.
\end{enumerate}

At each step the fractional size of $\cup_{S \in \cS} S$ grows by at least $1/k^{11}$, therefore the procedure must end in $k^{11}$ steps, therefore $m \leq k^{11}$. 

\paragraph{Union Bound:} It is enough to prove that none of the sets $S_1, \ldots, S_m \in \cS$ change by an additive factor $1/k^{22}$. This is because for all $g$:
\[\Agr_\eta(g) = (\Agr_\eta(g)\cap S_1) \cup \ldots \cup (\Agr_\eta(g)\cap S_m) \cup (\Agr_\eta(g)\setminus \cup_{S \in \cS} S),\]
where $|\Agr_\eta(g)\setminus \cup_{S \in \cS} S| \leq 1/k^{11}$ by the cover property. If none of the sets $S_i$ change by an additive factor of $1/k^{22}$ then $|\Agr_\eta(g)|$ can shrink by at most $k^{11}\cdot 1/k^{22}+1/k^{11} \ll 1/k^{10}$. 

Now note that the set $\Agr_\eta(g)\setminus \cup_{S \in \cS} S$ can grow by an additive factor of at most $1/k^{12}$ on $\cC(d(1-\beta))$ -- if inside some $s \in \cC(d(1-\beta))$ this set is of size $\gamma$ then it must have size at least $\gamma(1-\beta)^k$ on $\cC(k)$. Therefore if the original size on $\cC(k)$ was $\delta$ then $\gamma \leq \delta/(1-1/k)$ and therefore the growth in size is at most $\delta/k$ which is less than $1/k^{12}$ since $|\Agr_\eta(g)\setminus \cup_{S \in \cS} S| \leq 1/k^{11}$. Therefore $|\Agr_\eta(g)|$ grows by at most $1/k^{11}+1/k^{12} \ll 1/k^{10}$. 

So let us bound the probability that all of the sets $S_i$ do not change in size by too much.
To bound the probability for one set we use a concentration inequality:
\[\Pr_{s \sim X(d(1-\beta))}[|\E_{t \subset_k s}[\one[t \in S_i]] -\delta_i| \geq \frac{1}{k^{22}}] \leq \exp\left(-\frac{d}{k}\cdot\frac{1}{k^{22}}\cdot\log(1/k^2)\right),\]
where $\delta_i = |S_i|/|\cC(k)|$.

If $d \gg k^{23}\text{polylog}(k)$ then, the above is smaller than $1/k^{21}$, therefore we can union bound over all the sets to get that none of them jumps w.p. $1-1/k^{10}$.
\mitali{If instead of Chernoff we use sampling we need $d \gg k^{44}$.}

\end{proof}






\subsection{Codifying the lists - OLD}

We now note that each of the lists might be really large, but one can settle for approximate equality between the lists and the $k$-sets contained in it, to get a bounded list with large distance. We do this by throwing out small distance functions in the list, and noting that two functions with large distance cannot agree with many common $k$-sets. 

\begin{lemma}[Pruning the lists]
Show that keeping large distance functions preserves the list agreement acceptance probability.    
\end{lemma}

Once we have large distance one can show that the list cannot be of large size, since each element of the list agrees with $\geq \eps$-fraction of $k$-sets below it.

\begin{lemma}[Bounding list size]
The list can be of size $\leq O(1/\eps)$.    
\end{lemma}


\begin{lemma}[List agreement]
If agreement test on $X(k)$ passes with probability $\eps$ then the list agreement test on $X(d)$ passes with probability $1-\tau$ for $d=??$ and $\tau = o_k(1)$.    
\end{lemma}

\begin{proof}
Combining the above lemmas we finish the proof.
\end{proof}



Choose parameters $\tau \ll \eta_1 \ll \ldots \ll \eta_L \ll 1/L$. Use the following algorithm to codify the lists:

\begin{algorithm-thm}[]\label{alg:j} 
Input, output

\begin{enumerate}
\item Set $i=1$. 
\item 
\begin{compactenum}
\item 
\item Increment $j$.
\end{compactenum}
\item 
\end{enumerate}
\end{algorithm-thm}

After one iteration, 




\begin{lemma}\label{lem:conn-comp}
Distance vectors are almost equal across most of the edges.
\end{lemma}


\begin{lemma}
Can reduce lists to functions    
\end{lemma}

\begin{proof}
Since distance vectors are almost equal random threshold doesn't fall in the $\nu$ interval. So distance graphs are the same across most edges. On these edges picking one function in each component keeps list size the same across the edge and approximate agreement test is passed. To see this, assume $f_1$ was matched to $f'_1$ in the original test. Let $G_1$ and $G'_1$ be the strings that are chosen from the components of $f_1,f'_1$ respectively. We know that $\Delta_{A \cap A'}(f_1, G_1) \approx \Delta(f_1, G_1) \leq \eta_i$ and same for $f'_1,G'_1$. Additionally since the test passes on $(A,A')$, $\Delta(f_1, f'_1) \approx 0$, therefore by the triangle inequality we have, $\Delta(G_1, G'_1) \leq \Delta(G_1,f_1) +\Delta(f_1,f'_1)+ \Delta(f'_1, G'_1)$. 
\end{proof}


\subsubsection{Functions with largish-agreement do not jump}
In this section we prove that with high probability over $s \sim \cC(d)$ no function which has agreement in $[\delta^{10}, \delta - \delta^{10}]$ can jump to agreement $\delta$ inside $s$.

\begin{lemma}\label{lem:small-agr-jump}
    
\end{lemma}


We first prove some preliminary claims that we will use throughout.

\begin{claim}[Small Cover with large distance]\label{claim:small-cover}

\end{claim}


\begin{lemma}[Creating a gap]
There exists a set $\cF$ of functions $f: [d] \rightarrow \{0,1\}$ and parameters $\delta(\epsilon), r$ such that:
\begin{enumerate}
    \item Every function $f \in \cF$ has large agreement with $A$: $\agr(f,A) \geq \delta$.
    \item Every pair of functions $f, g \in \cF$ have large distance: $\Delta(f,g) \geq 10r$.
    \item $\cF$ is a cover of functions with large agreement: If $f'$ is such that $\agr(f') \geq \delta-\delta^{10}$ then there exists an $f \in \cF$ such that $\Delta(f,f') \leq r$.
\end{enumerate}
\end{lemma}

We now use the concentration inequality to show that for most $a$'s in $X(cd)$ no function with agreement in $[\delta^{10}, \delta-\delta^{10}]$ can jump to agreement $\delta$, for $c$ sufficiently large. We first use the small cover property to say that all such functions lie in an $R$-ball around some fixed $1/\delta^{10}$ functions. Then we use chaining to show that with high probability no function in an $R$-ball can jump to agreement inside a lower set in $\cC(cd)$.

\begin{lemma}
Let $\beta, \delta, \ldots$ satisfy??
Let $F$ be a global function such that all the global functions in its $R$-ball have agreement at most $\delta - \delta^{10}$. Then with high probability over $\cC(cd)$ all of these functions have agreement at most $\delta$:
\[\Pr_{s \sim \cC(cd)}[] \leq \tau.\]
\end{lemma}


\begin{proof}
Without loss of generality let $F$ be the all $0$s function. Let $\cB_R(F)$ denote the $R$-ball of functions around $F$, where we drop $R,F$ from the notation and let $\cB$ denote the $R$-ball around $0^d$. Let the $1$-set of a function $1(f) \subseteq [d]$ denote the set of coordinates where some function $f$ is $1$.

We will show that we can build a small $\gamma$-net for the agreement sets of the functions in $\cB$:  for all $g \in \cB$ there exists a function $f \in \cF$ such that $\Agr(g) \setminus \Agr(f)$ is of size at most $\gamma$. In fact, our net will be pretty simple: we will build a subset $C \subset [d]$ and let $\cF$ be the set of functions in $\cB$ whose $1$-sets are completely contained in $C$. In this case it suffices to check how the agreement set of $g$ compares with the projection of $g$ onto $C$, i.e. the function $g|_{C}$ which is defined as $g$ on $C$ and $0$ otherwise.

\paragraph{Construction of a $\gamma$-net for agreement sets of $\cB$:}
We first show how to build a $\gamma$-net of size $\exp(Rd\log(1/\gamma))$. We use the following algorithm:
\begin{enumerate}
\item Initialize $C = \phi$. 
\item While there exists $f \in \cB$ such that $|\Agr(f) \setminus \Agr(f|_C)| > \gamma$:
\begin{enumerate}
    \item Choose an arbitrary such function $f$.
    \item $C \leftarrow C \cup 1(f)$. 
\end{enumerate}
\item Output $C$.
\end{enumerate}
We will first show that this algorithm terminates in $1/\gamma$ steps. Let us consider the $i^{th}$-iteration where $\cF = \{g \in \{0,1\}^d: 1(g) \subset C \text{ and } |1(g)| \leq R\}$. Let the set $\Agr(\cF)$ be the union of all the agreement sets of functions in $\cF$. At the $i^{th}$-iteration suppose $f$ is such that $|\Agr(f) \setminus \Agr(f|_C)| > \gamma$. Now note that every $s \in \Agr(f) \setminus \Agr(f|_C)$ must contain some element from the set of coordinates $1(f)\setminus C$ since otherwise it is also satisfied by $f|_C$. This also means that $s \notin \Agr(\cF)$, since every $g \in \cF$ is $0$ on $1(f) \setminus C$. Therefore by adding the set $1(f)$ to $C$ and considering the corresponding family $\cF'$, the set $\Agr(\cF')$ grows by at least $\gamma$ in fractional size. Therefore this algorithm needs to conclude in $\lceil 1/\gamma \rceil$ steps.

We can now check that the set obtained by the algorithm has size at most $Rd\lceil 1/\gamma \rceil$. At each iteration we add $1(f)$ for $f \in \cB$ therefore $|C|$ increases by at most $R$. Therefore the functions in the cover are at most ${Rd\lceil 1/\gamma \rceil \choose Rd} = \exp(Rd\log(1/\gamma))$.

\paragraph{Chaining:}
Let us now define some parameters required for chaining. Let $m = ??$ and define the parameters: 
\[\gamma_0 = \delta-\delta^{10}, \gamma_1 =\delta^{11}, \gamma_2 = \delta^{22}, \ldots, \gamma_m = \delta^{11m},\] 
\[\delta_0 = \delta - \frac{1}{2}\delta^{10}, \delta_1 = \delta^{10}/4, \delta_2 = \delta^{10}/8, \ldots, \delta_m = \delta^{10}/2^{m+1}.\] 
\mitali{define the last parameter and $m$ such that the probability of jump is $0$}

For $i=1$, let $C_1$ and the corresponding family of functions $\cF_{1}$ be the $\gamma_1$-net of the agreement sets of $\cB$ defined above. By running the algorithm first for $\gamma_1$, we obtain $C_1$ and $\cF_{1}$, then for the parameter $\gamma_2$ we start the algorithm with the set $C_1$ and continue the iteration but with $\gamma_2$, so that we obtain $C_2 \supseteq C_1$ and $\cF_2 \supseteq \cF_1$. We go on like this for $\gamma_3$ and so on until we obtain the nested $\gamma$-nets for $\cB$: $C_1 \subseteq C_2 \subseteq \ldots \subseteq C_m$ and $\cF_1 \subseteq \cF_2 \subseteq \ldots \subseteq \cF_m$. One can check that for each $i$, $|C_i| \leq R\gamma_i$ and $|\cF_i| \leq \exp(Rd\log(1/\gamma_i))$. By the net-property we have that for all $g \in \cB$, $|\Agr(g) \setminus \Agr(g|_{C_i})| \leq \gamma_i$.

We now prove that w.h.p. over $s \sim \cC(cd)$ no function in $\cB$ jumps to agreement $\delta$. As is the case in chaining, we write the agreement set of a function $g \in \cB$ as:
\[\Agr(g) = \Agr(g|_{C_1}) \cup (\Agr(g|_{C_2}) \setminus \Agr(g|_{C_1})) \cup \ldots \cup (\Agr(g) \setminus \Agr(g|_{C_m})).\]

We first note that to say that $\mu_s(\Agr(g)) \leq \delta$ it suffices to prove that the size of the $i^{th}$-set in the decomposition above does not jump to $\delta_i$ for most $s \sim \cC(cd)$:
\begin{align*}
\mu_s(\Agr(g)) &\leq \mu_s(\Agr(g|_{C_1}))+ \ldots+ \mu_s(\Agr(g|_{C_{i+1}}) \setminus \Agr(g|_{C_i})) + \ldots \\
&< \delta - \frac{\delta^{10}}{2} + \frac{\delta^{10}}{4} + \ldots + \frac{\delta^{10}}{2^{m+1}} \\
&< \delta.
\end{align*}

Let us therefore show that for $i \geq 1$ w.h.p over $s$, for all $g \in \cB$ the $i^{th}$-set in the decomposition is of size at most $\delta_i$ inside $s$. Then we will union bound over the events to finish the proof. 
\paragraph{Bounding the probability for the $0^{th}$ term:}
The $0^{th}$ term $\Agr(g|_{C_1})$ is of size $\leq \gamma_0$ by assumption. The number of such sets when we range over $g \in \cB$ is at most $|\cF_1|$ since each function $g|_{C_1}$ belongs to $\cF_1$. By a union bound over $\cF_1$ we therefore get that the probability that any of these sets jumps from size $\gamma_0 \rightarrow \delta_0$ is small:
\begin{equation}\label{eq:chaining1}
\Pr_{s \in \cC(cd)}[\exists g \in \cB \text{ s.t. } \mu_s(\Agr(g|_{C_1})) \geq \delta_0] \leq |\cF_1| \cdot\exp\left(-\frac{d}{k}\log(1/\beta)\log(\delta_0/\gamma_0)\right) \leq \exp\left(-\frac{d}{k}\poly(1/\delta)\right),    
\end{equation}
where we used the concentration inequality (Lemma~\ref{lem:concentration}) proved earlier and simplified using $|\cF_1| \leq \exp(Rd\log(1/\delta))$, $R = O(\poly(1/\delta)/k)$ and $\beta \leq \exp(-\poly(1/\delta))$.

\paragraph{Bounding the probability for the $i^{th}$ term for $1 \leq i < m$:}
The $i^{th}$-set for $g$ is $(\Agr(g|_{C_{i+1}}) \setminus \Agr(g|_{C_i}))$. First note that this is a set of size at most $\gamma_i$ for all $g \in \cB$ by the net-property of $C_i$ applied on $g|_{C_{i+1}}$. Also note that the number of such sets when we range over all $g \in \cB$ is at most $|\cF_{i+1}|\cdot|\cF_{i}|$, since each function $g|_{C_i}$ belongs to $\cF_i$. By a union bound over the sets of the form $\Agr(f_1) \setminus \Agr(f_2)$ for $f_1 \in \cF_{i+1}$ and $f_2 \in \cF_i$ we get the probability that any of these sets jump in size inside $s$ is small:
\begin{align}
\Pr_{s \in \cC(cd)}[\exists g \in \cB \text{ s.t. } \mu_s(\Agr(g|_{C_{i+1}}) \setminus \Agr(g|_{C_{i}})) \geq \delta_i] &\leq |\cF_{i+1}| \cdot |\cF_i| \cdot \exp\left(-\frac{d}{k}\log(1/\beta)\log(\delta_i/\gamma_i)\right) \nonumber\\
&\leq \exp\left(-\frac{d}{k}\poly(1/\delta)\right).\label{eq:chaining2}
\end{align}
where to bound the probability of one term we used Lemma~\ref{lem:concentration} and then simplified using $|\cF_i| \leq \exp(Rd\log(1/\delta^{11i}))$, $R = O(\poly(1/\delta)/k)$ and $\beta \leq \exp(-\poly(1/\delta))$.

\paragraph{Bounding the probability for the $m^{th}$ term:}

\mitali{use that Chernoff gives 0 probability of jumping}


Adding up the terms in \eqref{eq:chaining1,eq:chaining2,eq:chaining3} we get that w.h.p. none of the terms in the decomposition jump from $\gamma_i$ to $\delta_i$ thus completing the proof of the lemma:
\[\Pr_{s \in \cC(cd)}[\exists g \in \cB \text{ s.t. } \mu_s(\Agr(g) \geq \delta] &\leq \sum_{i = 1}^m \Pr[] \nonumber\\
&\leq \exp\left(-\frac{d}{k}\poly(1/\delta)\right).\]

\end{proof}


\begin{lemma}[Concentration on the complete complex]\label{lem:concentration}
\mitali{not needed now}
Let $F$ be a $[-1,1]$-function on $\cC(k)$ with $\E[F^2] = \gamma$ and let $c = 1-\beta$ for a fixed constant $\beta \in (0,1)$. We have that,
\[\Pr_{s \sim \cC(cd)}[\E_{t \subset_k s}[F(t)] \geq \gamma'] \leq \exp\left(-\frac{d}{k}\log(\gamma'/\sqrt{\gamma})\log(1/\beta)\right).\]
%Furthermore, \mitali{say that when $\gamma$ is very small the probability of jump is $0$.}
\end{lemma}

\begin{proof}
Given $q \in (0,1)$, let $\mu_q$ be the distribution where $b = 1$ w.p. $q$ and $0$ otherwise and $\mu_q^{\otimes d}$ be the corresponding product distribution on $\cube$. It will be useful for us to prove an analogue of the lemma on $\cube$ using the product measure $\mu_c^{\otimes d}$. So let us define an extension of $F$ on $\cube$:
\[f(x) = \begin{cases} 
0 ~~~~~~~~~~~~~~~~~~~~ \text{ if } |x| < k, \\
F(x) ~~~~~~~~~~~~~~~ \text{ if } |x| = k, \\
\E_{t \subset_k x}[F(t)] ~~~~~ \text{ otherwise,}
\end{cases}
\]
where $|x|$ denotes the Hamming weight of $x$. Now, instead of bounding the probability that $\E_{t \subset_k x}[F(t)]$ deviates, let us again use the product measure $D(x)$ defined in the natural way as:
\[y_i = \begin{cases} 
0 ~~~~~~~~~~~~~~~~~~~~ \text{ if } x_i = 0, \\
1 ~~~~~~~~~~~~~~~ \text{ w.p. } \frac{p}{c} \text{ if } x_i = 1 \\
0~~~~~~~~~~~~~~~~~ \text{ w.p. } 1-\frac{p}{c} \text{ if } x_i = 1,
\end{cases}
\]
where $p$ is set to be $2k/d$ and each bit $y_i$ is chosen independently as above. Note that $y$ is always a subset of $x$ and when $|x| = cd$ then in expectation $y$ has size $2k$, and furthermore it has size at least $k$ w.h.p. We will prove that:
\begin{equation}\label{eq:cube}
\Pr_{x \sim \mu_c^{\otimes d}}[\E_{y \sim D(x)}[f(y)] \geq \gamma'] \leq \exp\left(-\frac{d}{k}\log(\gamma'/\gamma)\log(1/\beta)\right).    
\end{equation}

It is easy to see why the lemma follows from the above.

\paragraph{\eqref{eq:cube} $\Rightarrow$ Lemma:}
We have that w.p. at least $\Omega(1/\sqrt{d})$, $|x| = cd$ for $x$ drawn from $\mu_c^{\otimes d}$. Therefore \eqref{eq:cube} holds even when $x \sim \cC(cd)$:
\begin{equation}\label{eq:cube2}
\Pr_{x \sim \cC(cd)}[\E_{y \sim D(x)}[f(y)] \geq \gamma'] \leq \exp\left(-\frac{d}{k}\log(\gamma'/\gamma)\log(1/\beta)\right),    
\end{equation}
where we have multiplied the probability in \eqref{eq:cube} by $O(\sqrt{d})$ and used that $d \gg k$.

Therefore fix an $x$ with $|x| = cd$. We can use a Chernoff bound to get that $y \sim D(x)$ will be of size $\geq k$ w.h.p:
\[\Pr_{y \sim D(x)}[\sum_{i: x_i = 1}y_i < k] \leq \exp(-k).\]

\begin{align*}
\E_{y \sim D(x)}[f(y)] &= \sum_{i \geq k} \Pr_{y \sim D(x)}[|y| = i]\E_{y \sim D(x)}[f(y)~|~ |y| = i] + \Pr_{y \sim D(x)}[|y| < k]\E_{y \sim D(x)}[f(y)~|~ |y| < k] \\
&= \sum_{i \geq k} \Pr_{y \sim D(x)}[|y| = i]\E_{\substack{y \subset_i x \\ t \subset_k y}}[F(t)] \\
&= \Pr_{y \sim D(x)}[|y| \geq k]\E_{t \subset_k x}[F(t)] \\
&\geq (1-\exp(-k))\E_{t \subset_k x}[F(t)].
\end{align*}

Combining with~\eqref{eq:cube2} we therefore get that,
\begin{equation}\label{eq:cube3}
\Pr_{x \sim \cC(cd)}[\E_{t \subset_k x}[F(t)] \geq \frac{\gamma'}{(1-\exp(-k))}] \leq \Pr_{x \sim \cC(cd)}[\E_{y \sim D(x)}[f(y)] \geq \gamma'] \leq \exp\left(-\frac{d}{k}\log(\gamma'/\gamma)\log(1/\beta)\right),
\end{equation}
thus completing the proof of the Lemma given~\eqref{eq:cube}.

Let us now prove~\eqref{eq:cube}.

\paragraph{Proof of~\eqref{eq:cube}:}
For $q \in (0,1)$ and $S \subseteq [n]$, let $\Chi^q_S$ denote the standard $q$-biased character on $\{0,1\}^n$. 

Let us now use the operator $T^{p \rightarrow c}: L_2(\{0,1\}^n, \mu_p^{\otimes n}) \rightarrow L_2(\{0,1\}^n, \mu_c^{\otimes n})$ from~\cite{keevash2021global} defined as: $T^{p \rightarrow c}f(x) = \E_{y \sim D(x)}[f(y)]$. Therefore it suffices to bound the probability that $T^{p \rightarrow c}f(x)$ is large.

Firstly using Markov's inequality we get that for all $m \in \nn$, 
\begin{equation}\label{eq:markov}
\Pr_{x \sim \mu_c^{\otimes d}}[|T^{p \rightarrow c}f(x)| \geq \gamma'] \leq \frac{\E_{x \sim \mu_c^{\otimes d}}[|T^{p \rightarrow c}f(x)|^m]}{(\gamma')^m} \leq \frac{\gamma^{m/2}}{(\gamma')^m}.    
\end{equation}
We can now bound the RHS above using hypercontractivity. Let us write $f$ in its $p$-biased Fourier representation as $f = \sum_S \hat{f}(S)\Chi_S^p$. Let $g = \sum_S \hat{f}(S)\Chi_S^c$ and  $\rho = \sqrt{\frac{p(1-c)}{c(1-p)}}$. We can use Lemma III.3.3 from~\cite{keevash2021global} to get that,
\[T^{p \rightarrow c}\Chi_S^p = \sqrt{\rho}^{|S|}~\Chi_S^c,\]
therefore:
\[T^{p \rightarrow c}f = T_{\sqrt{\rho}}g,\]
where $T_{\sqrt{\rho}}$ is the usual noise operator. Using hypercontractivity for the $c$-biased distribution~\ref{lem:hypercontractivity} we get that for $m \leq ?$:
\[\E_{x \sim \mu_c^{\otimes d}}[g(x)^m]^{1/m} \leq \E_{x \sim \mu_c^{\otimes d}}[g(x)^2]^{1/2} = \sum_S \hat{f}(S)^2 = \E_{y \sim \mu_p^{\otimes d}}[f(y)^2]^{1/2}.\]

Using the definition of $f$ we get, 
\begin{align*}
\E_{y \sim \mu_p^{\otimes d}}[f(y)^2] &= \sum_{i \geq k}\Pr_{y \sim \mu_p^{\otimes d}}[|y| = i] \E_{y \sim \mu_p^{\otimes d}}[f(y)^2~|~|y| = i] + \Pr_{y \sim \mu_p^{\otimes d}}[|y| < k] \E_{y \sim \mu_p^{\otimes d}}[f(y)^2~|~|y| < k]  \\
&= \sum_{i \geq k}\Pr_{y \sim \mu_p^{\otimes d}}[|y| = i] \E_{y \sim \cC(i)}[\E_{t \subset_k y}[F(t)]^2] \\
&\leq \sum_{i \geq k}\Pr_{y \sim \mu_p^{\otimes d}}[|y| = i] \E_{t \sim \cC(k)}[F(t)^2] \\
&\leq \gamma.
\end{align*}
\end{proof}


%%%%%%%%%%%%%Short-list argument%%%%%%%%%%
\begin{lemma}[Short list with gap]\label{lem:gap}
Let $k \gg 1/\eps_0$, $t = ??$, $\delta = \eps_0 - \eps_0^{18}$. Algorithm~\ref{algo-gap} outputs a list $L = \{f_{i_1},\ldots,f_{i_m}\}$ for $i_j \in \{0,\ldots,\lfloor1/\delta^{80}\rfloor\}$
and a function $G$  with the following properties:
\begin{enumerate}
    \item $L$ is of size at most $2/\delta_0$.
    \item $\agr_t(f_i, F) > \delta$.
    \item For all $g$, $\agr_{t}(g, G) < \delta - \delta^{20}$.
    \item If $g$ on $s \in X(d/2)$ satisfies that $\Delta(g, f_i|_s) > \Omega(t/k)$ and $\agr_t(g,G|_s) < \delta -\delta^{100}$, then $\agr_t(g, F|_s) < \delta$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let us start by showing that the algorithm terminates in $< m_0$ steps.

\paragraph{Proof of (1)}: We will show that the algorithm terminates in $m_0$ steps. Suppose for the sake of contradiction that it does not and consider the $m_0^{th}$ step. At this iteration $\delta > \eps_0 - 2\eps_0^{19}$ and $t <\exp(1/\eps_0)$. Let $\cR \subseteq \cC(k)$ be the $k$-sets that have been randomized in the algorithm so far, so $|\cR| \geq \eps_0 {d \choose k}$. By a standard Chernoff we can prove that every function $g$ satisfies:
\[\Pr\left[\frac{|\Agr_t(g) \cap \cR|}{|\cC(k)|} > k \cdot \frac{k^t}{2^k}\right] \leq \exp(-\eps_0 d^k). \mitali{CHECK}\]
Therefore by a union bound we get that for all functions on $[d]$ ($2^d$ many) the above holds. Hence at each iteration of the algorithm the $k$-sets found do not intersect much with the previous ones and cover at least $\delta - o(1) \gg \eps_0/2$-fraction of $\cC(k)$ not covered before. Therefore the fraction of $\cC(k)$ covered is at least $(\delta-o(1))\cdot m_0 \gg 1$ which is a contradiction since
the fraction of $\cC(k)$ covered at any point can be at most $1$.

\paragraph{Proof of (2):} Let $\delta_{m-1}, t_{m-1}$ be the values of $\delta$ and $t$ in the final iteration. 
(2)  follows immediately given that the algorithm terminates in $m_0$ steps and at each step in the while loop we find a function with $\agr_{t_{m-1}}(f, F) \geq \agr_{t_{m-1}}(f, \widetilde{F}) > \delta_{m-1} > \eps_0 - \eps_0^{18}$.

\paragraph{Proof of (3):} This follows immediately from the fact that the algorithm exits the while loop.

\paragraph{Proof of (4):} Let $\cR$ be all the $k$-sets randomized by the algorithm inside $s$ when it terminates.
If $g$ and $f_i|_s$ are $\eta$-far for $\eta > \Omega(t/k)$ then $|\Agr_t(g, F|_s) \cap \Agr_t(f_i|_s, F|_s)| < \eps_0^{102}$, therefore $|\Agr_t(g, F|_s) \cap \cR| < 2\eps_0^{101}$. 
Since $|\Agr_t(g, F|_s) \cap \overline{\cR}| = |\Agr_t(g, G|_s) \cap \overline{\cR}| < \delta-\delta^{100}$, so overall we get $|\Agr_t(g, F)| < \delta-\delta^{100} + 2\eps_0^{101} < \delta$.
\end{proof}








%%%%%%%%%%%%%%%%%%%%%%%%%Agreement sets don't jump%%%%%%%%%%%%


\begin{mdframed}
\begin{algorithm}[Short list with gap]\label{algo-gap} \mbox{}
\begin{description}
\item[Input:] $F: \cC(k) \rightarrow \{0,1\}^k$.
\item [Output:] List of functions $\{f_1,\ldots,f_m\}$ from $[d] \rightarrow \{0,1\}$.
\item [Operation:]\mbox{}
\begin{enumerate}
    \item Set $t = u_1(\alpha_0,0)$, $\delta = u_2(\eps_0)$, $\widetilde{F} = F$, List $L =\phi$.
    \item While there exists $f$ with $\agr_t(f, \widetilde{F}) > \delta$: 
    \begin{itemize}
        \item Add $f$ to list $L$.
        \item Randomize $F$ on $k$-sets $A$ in $\Agr_t(f)$.
        \item $\delta \leftarrow \delta-\delta^{20}$ and $t \leftarrow 2u(\alpha_0, 1/t)$.
    \end{itemize}
    \item Output $L$ and $\widetilde{F}$.
\end{enumerate}
\end{description}
\end{algorithm}
\end{mdframed}

%%%%%%Modified Agreement tests on Johnson%%%%%%%%

We then consider the following modified agreement test for the purposes of our proof in Section~\ref{sec:core-jump}, where $F: \cC(k) \rightarrow \{0,1\}^k$ and $f: [d] \rightarrow \{0,1\}$.

\begin{mdframed}
\begin{agr-test}[$F,f, k, d, \alpha,\beta, R$]\label{agr-test-modified}\mbox{}
\begin{enumerate}
    \item Choose random $A, A' \subset_k [d]$ s.t. $|A \cap A'| = \alpha k$.
    \item Choose random $B \sim \mu_{\beta}([d])$.
    \item Accept if $F[A]|_{A \cap A' \cap B} = F[A']|_{A \cap A' \cap B}$ and $F[A] =_{<R} f[A]$.
\end{enumerate}
\end{agr-test}
\end{mdframed}

When this test passes we can show that there must be a function $g$ that is close to $f$ and has large global agreement with $F$.

\begin{theorem}[Soundness of Agreement Test~\ref{agr-test-modified}]\label{thm:agr-modified}
For every $\alpha, \beta \in (0,1)$, there exist $k_0(\alpha,\beta) \in \N$, $\delta_0(\alpha,\beta) \in (0,1)$, $u = u_2(\alpha,\beta) \in \N$ such that for all $k_0 \leq k \ll d, \delta \geq \delta_0$ the following holds. If the Agreement-Test~\ref{agr-test-modified} ($F,f,k,d,\alpha,\beta, R$) with probability $\delta$, then there exists $g$ such that $\Delta(f,g) < R+u/k$ and,
\[\Pr_{A \sim \cC(k)}[F[A] =_{<u} g(A)] \geq \delta',\]
where $\delta'$ is a growing function of $\delta$. 
\end{theorem}

\begin{proof}
This is proved using Theorem~\ref{thm:agr-basic}. 
\end{proof}







\subsubsection{Agreement sets do not jump}
Fix $\alpha_0 = \eps_0^{1000}$ as the intersection size of the agreement test throughout (no need to set it differently anywhere currently). Let $u(\alpha,\beta)$ be the disagreement function from Lemma~\ref{thm:agr-basic}.

\begin{lemma}[No jump]\label{lem:no-jump}
Given $T = \max(u(\alpha_0, 1/t), ??)$ and a function $G: \cC(k) \rightarrow \{0,1\}^k$ such that, $\agr_{T}(g,G) < \delta - \delta^{18}$ for all $g$ on $[d]$ then:
\[\Pr_{s \sim \mu_{1/2}(d)}[\exists f, \agr_t(f|_s,G|_s) > \delta -\frac{\delta^{18}}{2}] \leq \gamma_1 + 2\gamma_2/\delta^{100}.\]
\end{lemma}


\mitali{In this lemma, get $T$ only a function of $t$ but $d/k$ can depend on $T, 1/R$}
\begin{lemma}\label{lem:core-jump}
Let $R \in (0,1)$ with $R > T/k$, $T = 2u(\alpha_0,1/t)$ and $f$ be a function on $[d]$. Suppose for all functions $g \in \cB_R(f)$, $\agr_T(g, G) < \delta-\delta^{18}$ and for all $g \in \cB_{10R}(f) \setminus \cB_R(f)$, $\agr_T(g,G) <\delta^{100}$ then,
\[\Pr_{s \sim \mu_{1/2}(d)}\left[\forall f' \in \cB_R(f) \text{ with } \agr_t(f'|_s, G|_s) > \delta - \frac{\delta^{18}}{2}\right] > 1-\gamma_2.\]
\end{lemma}

Given this lemma, we are ready to prove Lemma~\ref{lem:no-jump}.

\begin{proof}[Proof of Lemma~\ref{lem:no-jump}]
Consider the following algorithm that generates a list of functions $f_1, \ldots, f_m$ on $[d]$.
\begin{mdframed}
\begin{algorithm}\label{algo-gap} \mbox{}
\begin{description}
\item[Input:] $G: \cC(k) \rightarrow \{0,1\}^k$.
\item [Output:] List of functions $\{f_1,\ldots,f_m\}$ from $[d] \rightarrow \{0,1\}$.
\item [Operation:]\mbox{}
\begin{enumerate}
    \item Set $T,\delta$ as in Lemma~\ref{lem:no-jump}, $\widetilde{G} = G$, List $L =\phi$.
    \item While there exists $f$ with $\agr_T(f, \widetilde{G}) > \delta^{40}$:
    \begin{itemize}
        \item Add $f$ to list $L$.
        \item Update $\widetilde{G}$ by randomizing the $k$-sets $A$ in $\Agr_T(f, \widetilde{G})$.
    \end{itemize}
    \item Output $L$ and $\widetilde{G}$.
\end{enumerate}
\end{description}
\end{algorithm}
\end{mdframed}

As in the proof of Lemma~\ref{lem:gap} we can show that:
\begin{enumerate}
    \item $|L| \leq 2/\delta^{100}$. 
    \item All $g$ satisfy $\agr_T(g, \widetilde{G}) < \delta^{100}$.
\end{enumerate}
We omit the proof here since it is the same as that of Lemma~\ref{lem:gap}. We get the following:
\begin{enumerate}
    \item The Agreement-Test$(\widetilde{G}, k,d,\alpha,1/t)$ passes w.p. $<\delta^{50}$ by Theorem~\ref{thm:agr-basic}. 
    \item By sampling w.p. $1-\gamma_1$ on $s \sim X(d/2)$, the Agreement-Test$(\widetilde{G},k,d/2,1/t)$ passes w.p. $< 2\delta^{50}$ and call every such $s$ a good set.
    \item On every good $s$, all functions $g$ on $s$ satisfy $\agr_t(g,\widetilde{G}|_s) < \delta^{25}$ (since if not the agreement test would pass w.p. $>2\delta^{50}$).
    \item Furthermore on every good $s$, every function $g: s \rightarrow \{0,1\}$ with $\Delta(g, f_i|_s) > r = \Omega(T/k), \forall i \in [m]$ must satisfy $\agr_t(g, G|_s) < \delta - \frac{\delta^{18}}{2}$. 
    \begin{proof}
    Let $\cR_i$ be the $k$-sets that were randomized at the $i^{th}$ iteration of the algorithm. We know that $\cR_i \subseteq \Agr_T(f_i)$. By the distance of $g$ from $f_i|_s$, using Claim~\ref{claim:dist-vs-agr} we get $|\Agr_t(g, G|_s) \cap \cR_i| < \delta^{200}$ when $r = \Omega(T/k)$. This implies that $|\Agr_t(g, G|_s) \cap (\cup_i \cR_i)| < \delta^{100}$. We have that: 
    \begin{align*}
    \agr_t(g, G|_s) &= |\Agr_t(g, G|_s) \cap (\cup\cR_i)| + |\Agr_t(g, G|_s) \cap (\overline{\cup\cR_i})| \\
    &\leq \delta^{100} + \agr_t(g, \widetilde{G}) \leq 2\delta^{25}.    
    \end{align*}
    \end{proof}
    \mitali{apply Lemma~\ref{lem:core-jump} after merging balls and getting distance between balls}
    \item Now suppose for the sake of contradiction that w.p. $\gamma_1 + 2\gamma_2/\delta^{100}$ on $s \sim X(d/2)$ there exists a function $g_s$ with $\agr_t(g_s, G|_s) > \delta-\delta^{18}/2$. Since at most $\gamma_1$ $s$ are not good, $2\gamma_2/\delta^{100}$-fraction of these $s$'s are good and therefore by (4) above, we know that $g_s$ must be $R$-close to some $f_i|_s, i \in [m]$. 
    \item Therefore for at least $\gamma_2$-fraction of $s$, there exist $g_s$ that is $R$-close to $f_{i_0}$ for a fixed $i_0 \in [m]$, and $\agr_t(g_s, G|_s) > \delta - \delta^{18}/2$. Define $h(s)$ on $[d]$ as $g_s \circ f_{i_0}|_{\overline{s}}$. We have that $g_s = h(s)|_s$, and $\Delta(h(s), f_{i_0}) < R$. Hence we have a contradiction to Lemma~\ref{lem:core-jump}, and this finishes the proof. 
\end{enumerate}
\end{proof}


\subsubsection{Proof of Lemma~\ref{lem:core-jump}}\label{sec:core-jump}
Fix $R, t, T$ as in Lemma~\ref{lem:core-jump}. Without loss of generality, we can assume that $f$ is the all $0$'s function and use $\cB$ to denote $\cB_R(0)$ when the radius is clear from context. To prove this lemma, we will build a small $\gamma$-net for the agreement sets of the functions in $\cB$:  for all $g \in \cB$ there exists a function $f \in \cF$ such that $\Agr(g) \setminus \Agr(f)$ is of size at most $\gamma$. In fact, our net will be pretty simple: we will find a subset $C \subset [d]$ and let $\cF(C)$ be the set of functions whose $1$-sets are completely contained in $C$. In this case it suffices to check how the agreement set of $g$ compares with the projection of $g$ onto $C$, i.e. the function $g|_{C}$ which is defined as $g$ on $C$ and $0$ outside $C$.


\begin{lemma}[Finding Core Set]\label{lem:core-set}
We can find a set $C$ of size at most $\frac{RTd}{\gamma}$ such that for all $g \in \cB(0)$:
\[|\Agr_T(g) \setminus \Agr_T(g|_C)| \leq \gamma.\]
\end{lemma}

\begin{proof}
\mitali{change this proof}

To construct $C$ use the following algorithm:
\begin{enumerate}
\item Initialize $C = \phi$. 
\item While there exists $f \in \cB$ such that $|\Agr_T(f) \setminus \Agr_T(f|_C)| > \gamma$:
\begin{enumerate}
    \item Choose an arbitrary such function $f$.
    \item $C \leftarrow C \cup 1(f)$. 
\end{enumerate}
\item Output $C$.
\end{enumerate}
We will first show that this algorithm terminates in $T/\gamma$ steps. Let us consider the $i^{th}$-iteration where $\cF = \{g \in \{0,1\}^d: 1(g) \subset C \text{ and } |1(g)| \leq R\}$. Let the set $\Agr(\cF)$ be the union of all the agreement sets of functions in $\cF$. At the $i^{th}$-iteration suppose $f$ is such that $|\Agr(f) \setminus \Agr(f|_C)| > \gamma$. Now note that every $s \in \Agr(f) \setminus \Agr(f|_C)$ must contain some element from the set of coordinates $1(f)\setminus C$ since otherwise it is also satisfied by $f|_C$. This also means that $s \notin \Agr(\cF)$, since every $g \in \cF$ is $0$ on $1(f) \setminus C$. Therefore by adding the set $1(f)$ to $C$ and considering the corresponding family $\cF'$, the set $\Agr(\cF')$ grows by at least $\gamma$ in fractional size. Therefore this algorithm needs to conclude in $\lceil 1/\gamma \rceil$ steps.

We can now check that the set obtained by the algorithm has size at most $Rd\lceil 1/\gamma \rceil$. At each iteration we add $1(f)$ for $f \in \cB$ therefore $|C|$ increases by at most $R$.
\end{proof}

The following lemma is proved in the next section.
\begin{lemma}\label{lem:union-bound}
For all $T \in \N$, $C \subset [d]$, and $d/k \geq u(T,|C|,\gamma)$,
\[\Pr_{s \sim X(d/2)}[\forall f \in \cF(C), \agr_T(f|_s, G|_s) < \agr_T(f, G) + \gamma] \geq 1-o(1).\]
\end{lemma}


Using this we can complete the proof of Lemma~\ref{lem:core-jump}.

\begin{lemma}[Lemma~\ref{lem:core-jump} restated]
Let $T = 2u(\alpha_0,1/2t)$, $R \in (0,1)$ with $R > T/k$,  and $f$ be a function on $[d]$. Suppose for all functions $g \in \cB_R(f)$, $\agr_T(g, G) < \delta-\delta^{18}$ and for all $g \in \cB_{10R}(f) \setminus \cB_R(f)$, $\agr_T(g,G) <\delta^{100}$ then,
\[\Pr_{s \sim \mu_{1/2}(d)}\left[\forall g \in \cB_R(f) \text{ with } \agr_t(g|_s, G|_s) > \delta - \frac{\delta^{18}}{2}\right] > 1-\gamma_2.\]
\end{lemma}


\begin{proof}
Using Lemma~\ref{lem:core-set} we find a set $C$ of size at most $O(TRd/\delta^{100})$ such that for all $g \in \cB$:
\begin{equation}\label{eq:gamma-cover}
|\Agr_{T/2}(g) \setminus \Agr_{T/2}(g|_C)| \leq \delta^{100}.    
\end{equation}

Let $\cR$ be all $A \in \cC(k)$ with $\Delta(G[A]|_{\overline{C}}, 0) \leq T/2$. For all $g \in \cB$ write:
\[\Agr_{T/2}(g) = A_1(g) \sqcup A_2(g),\]
where $A_1(g) = \Agr_{T/2}(g) \cap \cR$ and $A_2(g) = \Agr_{T/2}(g) \setminus \cR$. To bound $\agr_t(g|_s, G|_s)$ we bound $|A_1(g)|_s|$ and $|A_2(g)|_s \cap \Agr_t(g|_s, G|_s)|$ separately.

\paragraph{Bounding size of $A_1(g)|_s$:}
We get that $A_1(g) \subseteq \Agr_{T}(g|_C)$. Let $h$ denote the function $g|_C$. This is because on $A \in \Agr_{T/2}(g)$, $\Delta(G[A]|_C,h[A]|_C) = \Delta(G[A]|_C,g[A]|_C) \leq \Delta(G[A],g) \leq T/2k$ and $A \in \cR$, $\Delta(G[A]|_{\overline{C}}, h[A]|_{\overline{C}}) = \Delta(G[A]|_{\overline{C}}, 0) \leq T/2k$, therefore giving us that for $A \in \cR \cap \Agr_{T/2}(g)$, \[\Delta(G[A],h[A]) = \Delta(G[A]|_C,h[A]|_C) + \Delta(G[A]|_{\overline{C}},h[A]|_{\overline{C}}) \leq T/k.\]

Using Lemma~\ref{lem:union-bound} we get that w.h.p. over $s \in X(d/2)$, for all $g \in \cB$,
\[|A_1(g)|_s| \leq \agr_{T}((g|_C)|_s, G|_s) \leq \agr_{T}(g|_C) + \delta^{100} \leq \delta-\delta^{18}+\delta^{100}.\]

\paragraph{Bounding size of $A_2(g)|_s \cap \Agr_t(g|_s, G|_s)$:}
$\cR$ contains the set $\Agr_{T/2}(g|_C)$ for all $g$, therefore \eqref{eq:gamma-cover} gives us that for all $g \in \cB$, $A_2(g) \leq \delta^{100}$. Randomize $G$ on $\cR$ to get $\widetilde{G}$. We know that $\agr_{T/2}(g, \widetilde{G}) \leq |A_2(g)|+o(1) \leq \delta^{100}+o(1)$ for all $g \in \cB_R(0)$. By the assumption in the lemma statement we also know that $\agr_{T}(g,G) \leq \delta^{100}$ for all $g \in \cB_{10R}(0) \setminus \cB_R(0)$, which then implies that $\agr_{T/2}(g, \widetilde{G}) \leq \delta^{100}$ for all $g \in \cB_{10R}(0)$. Consider the Agreement-Test~\ref{agr-test-modified}$(\widetilde{G},0,k,d,\alpha_0,1/2t,5R)$, where by definition $T/2 = u(\alpha_0,1/2t)$. If it passed w.p. $>\delta^{50}$, by Theorem~\ref{thm:agr-modified} we would get that there exists a function $g \in \cB_{5R+T/2k}(0) \subset \cB_{6R}(0)$ with $\agr_{T/2}(g) \geq \delta^{100}$. Since no such function exists we get that the test passes w.p. $<\delta^{50}$. By sampling we get that w.p. $1-o(1)$ over $s \in X(d/2)$ the Agreement-Test~\ref{agr-test-modified}$(\widetilde{G}|_s,0,k,d/2,\alpha_0,1/2t)$ also passes w.p. $<2\delta^{50}$. On such an $s$ we claim that all $g \in \cB_R(0)$ satisfy $\agr_t(g|_s, \widetilde{G}|_s) < \delta^{24}$. Assume for contradiction that this was not the case, i.e. for one such $s$ there is a function $g \in \cB_R(0)$ with $|\Agr_t(g|_s, \widetilde{G}|_s)| > \delta^{24}$. Since $\Delta(g,0) \leq R$, $\Delta(g|_s, 0|_s) \leq 2R$ and w.p. $1-\exp(-Rk) \geq 1-\delta^{24}/2$ over $A \sim \cC_s(k)$, $\Delta(g|_s[A], 0|_s[A]) \leq 4R$ by Claim~\ref{claim:dist-chernoff}. Therefore the set $S = \Agr_t(g|_s, \widetilde{G}|_s) \cap \one(A: \Delta(g|_s[A], 0|_s[A]) \leq 4R)$ has size at least $\delta^{24}/2$. Then by the expander mixing lemma (Claim~\ref{claim:exp-mixing}) we would get that:
\[\Pr_{\substack{A,A' \sim \cC_s(k) \\ |A \cap A'| =\alpha k}}[A \in S, A' \in S] \geq \frac{\delta^{48}}{4} - \frac{\alpha_0\delta^{24}}{2} \geq \delta^{49}.\]
On an edge $(A,A') \in S$, note that $|A \cap A'|\Delta_{A \cap A'}(\widetilde{G}[A],\widetilde{G}[A']) \leq 2t$. Therefore the random $B$ picked in 
Agreement-Test~\ref{agr-test-modified} lies completely in the positions where the two strings agree w.p. $\geq 1/e$ and that part of the test passes. The second condition of the test: $\widetilde{G}[A] =_{<5R} 0[A]$ is satisfied since on $A \in S$, $\Delta(\widetilde{G}[A],0[A]) \leq \Delta(\widetilde{G}[A],g[A])+\Delta(g[A],0[A]) \leq t+4R < 5R$. Therefore overall the Agreement-Test~\ref{agr-test-modified} passes w.p. $\geq \delta^{49}/e > 2\delta^{50}$, which is a contradiction. Therefore we get that on such good $s$, for all $g \in \cB_R(0)$, $|A_2(g)|_s \cap \Agr_t(g|_s, G|_s)| \leq |\Agr_t(g|_s, \widetilde{G}|_s)| \leq \delta^{24}$.

Combining the bound on $|A_1(g)|_s|$ with $|A_2(g)|_s \cap \Agr_t(g|_s, G|_s)|$ completes the proof to get that w.p. $1-o(1)$ on $s$, for all $g \in \cB_R(0)$, $\agr_t(g|_s, G|_s) \leq \delta-\delta^{18}/2$.

%Since ${A_2(g) \subseteq \Agr_T(g) \setminus \Agr_T(g|_C)}$ we get that $A_2(g) \leq \delta^{40}$. Therefore after randomization $\Agr_T(g) \leq \delta^{40}$ for all $g$. Therefore the $\beta$-agreement test for $\beta = 1/t$ passes w.p. $\leq \delta^{20}$ globally. Therefore on most $s$, all functions satisfy $\agr_t(f) \leq \delta^{10}$. This implies that $A_2(g) \cap \Agr_t(g)$ jumps to at most $\delta^{10}$, and $A_1(g) \cap \Agr_t(g)$ jumps to at most $\delta-\delta^5+\delta^{100}$ therefore $\agr_t(g)$ on most $s$ is at most $\delta$.
\end{proof}



\subsubsection{Proof of Lemma~\ref{lem:union-bound}: Bounding agreement sets of all functions in $\cF(C)$}
Given a core set $C$ with respect to the function all 0s (wlog), recall that $\cF(C)$ is the set of all functions $f$ that are $0$ on $\overline{C}$. We let $\cF$ denote $\cF(C)$. Let $\cC_{I,s}(k)$ denote the set of $k$-sets in $[d]$ that contain $I$ and are contained within $s$.


\begin{lemma}\label{lem:basic-sets}
For all $I,B$:
\[\Pr_{s \sim \cC(d/2)}[\mu_{I,s}(I,B) - \mu_I(I,B) > \gamma] \leq o(1).\]    
\end{lemma}

\mitali{define notation for absolute distance}



\begin{proof}[Proof of Lemma~\ref{lem:union-bound}]
Define the sets $S_{i,b}$ for $i \in C$ and $b \in \{0,1\}$ as follows:
\[S_{i,b} := \{A \subseteq \cC(k) \mid A \cap C = \{i\} \text{ and } \Delta(G[A]|_{i},b)+ \Delta(G[A]|_{A \setminus i}, 0) \leq T\},\]
and more generally for $I \subseteq_{\leq k} C$ and $B \in \{0,1\}^{|I|}$ define $S_{I,B}$ as:
\[S_{I,B} := \{A \subseteq \cC(k) \mid A \cap C = I \text{ and } \Delta(G[A]|_I,B)+\Delta(G[A]|_{A \setminus I},0) \leq T\}.\]

Note that the sets $S_{I,B}$ are disjoint for different $I$ and moreover for all $f \in \cF$:
\[\Agr_T(f) = \sqcup_{I \subseteq C} S_{I, f|_I}.\]
Let $\mu(I,B)$ denote the fractional size of $S_{I,B}$ in $\cC(k)$. By the disjointedness of $S_{I,B}$'s we get that,
\[\agr_T(f) =  \sum_{I \subseteq C} \mu(I, f|_I) = \sum_{j=0}^k \agr^{=j}_T(f),\]
where $\agr_T^{=j}(f)$ as $\sum_{\substack{I \subseteq C \\ |I|=j}} \mu(I,f|_I)$. 

For some $s \in X(d/2)$ let $\mu_s(I,B)$ denote the fractional size of $S_{I,B}$ in all $k$-sets contained in $s$ and let $\mu_{s}(I,B)$ denote the fractional size of $S_{I,B}$ inside all $k$-sets that are contained in $s$. As above we then get that:
\[\agr_T(f|_s) = \sum_{I \subset C \cap s} \frac{|S_{I,f|_I}|}{|\cC_s(k)|} = \sum_{I \subset C \cap s} \mu_s(I,f|_I).\]


\paragraph{Bounding $\agr^{=j}_T(f|_s)-\agr^{=j}_T(f)$ for $j \leq j_0$:}
Since the set $S_{I,B}$ lies completely in the link of $I$ (in the complete complex), let $\mu_{I}(I,B)$ and $\mu_{I,s}(I,B)$ denote the fractional size of $S_{I,B}$ inside $\cC_{I,[d]}(k)$ and $\cC_{I,s}(k)$ respectively.

Therefore for all $j \leq j_0 = \poly(|C|k/d)$ chosen so that $j_0 \ll k$ we get, 
\[\agr^{=j}_T(f) = \sum_{I \subseteq C: |I|=j} \left(\frac{k}{d}\right)^j \mu_{I}(I, f|_I),\] 
and
\[\agr^{=j}_T(f|_s) = \sum_{I \subseteq C \cap S: |I|=j} \left(\frac{2k}{d}\right)^j \mu_{I,s}(I, f|_I).\] 


Let upper bound: $\agr^{=j}_s(f) - \agr^{=j}(f)$. 
\begin{align*}
\agr^{=j}_s(f) - \agr^{=j}(f) &= \sum_{I \subset C \cap S:|I|=j}\left(\frac{2k}{d}\right)^j\mu_{I,s}(I,f|_I) - \sum_{I \subset C:|I|=j}\left(\frac{k}{d}\right)^j\mu_I(I,f|_I) \\
&= \left(\frac{k}{d}\right)^j (\sum_{I \subset C\cap S:|I|=j} 2^j\mu_{I,s}(I,f|_I) - \mu_I(I,f|_I) - \sum_{\substack{I \subset C,\\ I\not\subset C \cap S,\\|I|=j}} \mu_I(I,f_I)) \\
&= \left(\frac{k}{d}\right)^j (\sum_{I \subset C\cap S:|I|=j} (2^j-1)\mu_{I}(I,f|_I) - \sum_{\substack{I \subset C,\\ I\not\subset C \cap S,\\|I|=j}} \mu_I(I,f_I) + \sum_{I \subset C\cap S:|I|=j}\Delta_s(I,f|_I)), 
\end{align*}
where $\Delta_s(I,B) := \mu_{I,s}(I,B) - \mu_I(I,B)$. We will bound the two terms separately. Define the vector $r \in \{\pm 1\}^{|C|}$ as $r_i = 1$ if $i \in s$ and $-1$ otherwise. We can rewrite the first term as:
\[F_j(r) = \left(\frac{k}{d}\right)^j\sum_{I \subset C\cap S:|I|=j} (2^j-1)\mu_{I}(I,f|_I) - \sum_{\substack{I \subset C,\\ I\not\subset C \cap S,\\|I|=j}} \mu_I(I,f_I) = \left(\frac{k}{d}\right)^j\sum_{I \subset C:|I|=j} \mu_I(I,f|_I)(\prod_{i \in I}(1+r_i) - 1).\]
We have the following claim:
\begin{claim}\label{claim:second-moment}
\[\|F_j\|_2 \leq \exp(j)\sqrt{\frac{k}{d}}.\]
\end{claim}
Using this we can apply concentration for low-degree polynomials (Lemma~\ref{lem:conc-low-deg}) to get that:
\[\Pr_{r \sim \mu_{1/2}^{\otimes |C|}}[|F(r)| > t\|F\|_2] \leq \exp().\]


\paragraph{Bounding $\agr^{=j}_T(f|_s)-\agr^{=j}_T(f)$ for $j \geq j_0$:}

    
\end{proof}




%%%%%%%% Existence of sparse UG coboundary expanders
\subsection{Do Sparse UG Coboundary Expanders Exist?}\label{sec:cobdry-discussion}
This is perhaps the most evident question that arises out of our work. A recent work by Chapman and Lubotzky~\cite{ChapmanL} shows that there are $(m,r,\xi,c)$-UG coboundary expanders for $m=2$ and $r=1$ \footnote{Note that $r=1$ is the first non-trivial setting of parameters where coboundary expansion is not the same as spectral expansion.}, which opens up the possibility of constructing high-dimensional ($r \geq 2$) UG coboundary expanders. Below we discuss some details.

For simplicity let us first consider $r=1$ in Definition~\ref{def:ug_coboundary_expander_simplified}. In the literature, proving that a complex is an $(m,1,\xi,c)$ coboundary expansion consists of two steps: 
\begin{enumerate}
\item Proving ``cosystolic expansion'': This step shows that every $(1-\xi)$-triangle consistent UG instance on $G_1[X]$, is $(1-c)$-close to a UG instance that is consistent on \emph{all} triangles. That is, it is possible to change the permutations on $c$-fraction of the edges so that all triangles are consistent.
\item Proving ``vanishing cohomology'': This step shows that every UG instance that is $1$-triangle consistent has an assignment to $V(G_1[X])$ that satisfies all the edges of the UG instance. This step typically requires deep results from algebra and number theory.
\end{enumerate}

For $r=1$ or $G_1[X]$, there are some LSV complexes that are cosystolic expanders~\cite{KaufmanKazLub, EvraKaufman}, and additionally~\cite{KaufmanKazLub} showed that under a number theoretic conjecture of Serre, some LSV complexes have vanishing cohomology when $m=2$\footnote{These are also called $2$-dimensional coboundary expanders over $\F_2$.}. Recently, Chapman and Lubotzky~\cite{ChapmanL} showed an unconditional construction of sparse complexes with vanishing cohomology when $r=1$ and $m=2$. This along with a theorem of~\cite{EvraKaufman} implies that there are constants $\xi,c \in (0,1)$ such that there exist $(2,1,\xi,c)$-UG coboundary expanders. Lubotzky~\cite{personal} informed us that with more care this proof can be extended to work for all $m$, therefore showing that there are sparse complexes that are $(m,1,\xi,c)$-UG coboundary expanders.

%Together these two results imply that there are constants $\xi,c \in (0,1)$ such that for all $m$, there are sparse HDX that are $(m,1,\xi,c)$-coboundary expanders. 

This by itself is not enough to give us new direct product testers since our argument requires large (but constant) $r$. For higher $r$, one might be able to show that $G_r[X]$ has vanishing cohomology by a reduction to $r=1$. As for the cosystolic expansion, one can show that for some LSV complexes, $G_r[X]$ is a cosystolic expander when $\xi <\exp(-r)$. Our argument uses $\xi = \exp(-o(r))$ (Theorem~\ref{thm:stronger-coboundary_formal}), therefore we would need improved bounds than those currently known. We leave the investigation of both these questions to future work. A positive resolution of these questions would give constructions of sparse HDX that are also sufficiently strong high-dimensional UG coboundary expanders thus implying sparse direct product testers in the low soundness regime.
















